Decision-Focused Summarization

Relevance in summarization is typically defined based on textual information alone, without incorporating insights about a particular decision. As a result, to support risk analysis of pancreatic cancer, summaries of medical notes may include irrelevant information such as a knee injury. We propose a novel problem, decision-focused summarization, where the goal is to summarize relevant information for a decision. We leverage a predictive model that makes the decision based on the full text to provide valuable insights on how a decision can be inferred from text. To build a summary, we then select representative sentences that lead to similar model decisions as using the full text while accounting for textual non-redundancy. To evaluate our method (DecSum), we build a testbed where the task is to summarize the first ten reviews of a restaurant in support of predicting its future rating on Yelp. DecSum substantially outperforms text-only summarization methods and model-based explanation methods in decision faithfulness and representativeness. We further demonstrate that DecSum is the only method that enables humans to outperform random chance in predicting which restaurant will be better rated in the future.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

First paragraph: Motivate why we need summarization to support decision making

Second paragraph: explain why text-only summarization is insufficient

Third/fourth paragraph: introduce our components briefly, leverage a model, decision faithfulness, decision representativeness. Present the figure on which sentences are chosen to illustrate decision representativeness.

Fifth: explain the restaurant task, and key results from automatic Metrics

Sixth: explain human evaluation and suggest many future directions.


The main contributions are to \chenhao{this can stay, I think that NLP applications will particularly like such a bullet list.}

\begin{itemize}
    \item We propose a novel summarization task that emphasizes supporting decision making.
    \item We propose ``decision faithfulness'' and ``decision representativeness'' as important criterion for this task in addition to meaning diversity.
    \item Using Yelp future rating prediction as a testbed, we show that the proposed algorithm outperform prior approaches based on text summarization and explanation generation.
    \item We show that the proposed algorithm effectively support human decision making.
\end{itemize}

==> related_work.tex <==
\section{Related Work}

Our work is most relevant to query-focused summarization in the vast literature on summarization.


\para{Sentiment-/aspect-based summarization}
\begin{enumerate}
    \item A Sentimental Education: Sentiment Analysis Using Subjectivity
    Summarization Based on Minimum Cuts
    Bo Pang and Lillian Lee
    \item A Joint Model of Text and Aspect Ratings for Sentiment Summarization
    Ivan Titov
    Ryan McDonald
\end{enumerate}

\para{Query- and decision-based Summarization.}
\begin{enumerate}
    \item AFastSum:
    Fast and accurate query-based multi-document summarization
    Frank Schilder and Ravikumar Kondadadi
    \item Query-Focused Opinion Summarization for User-Generated Content
    Lu Wang1 Hema Raghavan2 Claire Cardie1 Vittorio Castelli3
    \item Focused Meeting Summarization via Unsupervised Relation Extraction
    Lu Wang Claire Cardie \joe{The "decision" in this paper is different from our definition.}
    \item Query-Based Summarization: A survey
    Mariana Damova1 , Ivan Koychev2*
    \item Text summarization as a decision support aidT Elizabeth Workman, Marcelo Fiszman  John F Hurdle 
\end{enumerate}
\chenhao{clinical decision support, evidence inference by Byron Wallace should go here too.}

\para{Content Diversity}
\begin{enumerate}
    \item A Class of Submodular Functions for Document Summarization
    Hui Lin Jeff Bilmes. one which encourages the summary to be
    representative of the corpus, and the other
    which positively rewards diversity.
\end{enumerate}

\para{Attribution methods.}

Our focus is on the behavioral outcome of the sentences, i.e., whether they would support human decision making by identifying relevant information for the decision. As a proxy, we find sentences that lead to the same decision for the model as the full text.
It is not critical that these sentences are actually the evidence used by the model.
\chenhao{this can be merged into method or in related work. depending on what our related work looks like later.}

\para{Summarization evaluation.}

\para{Forecasting.}




==> summary_pairs.tex <==




\begin{table*}[h!]
    \centering
    \small
    
\begin{tabular}{p{0.07\linewidth} | p{0.43\linewidth} | p{0.43\linewidth} | p{0.07\linewidth} }
        \toprule
        method &                                                                                                                                                                                                                                                                                                                                                                                                                               b1summary &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        b2summary &  correct \\
 \midrule
 random &                                        {\color{orange}$x_1$:}  I was impressed - not only was it fresh, but the bread was delicious. {\color{orange}$x_2$:}  All of the kids acted completely un interested in making sure we had what we needed. {\color{orange}$x_3$:}  My decision:  a turkey unwich. {\color{orange}$x_4$:}  The only thing that I was disappointed with {\color{orange}$x_5$:}  Now I crave sandwiches from there. &                                                                  {\color{orange}$x_1$:}  They cook the patties to pink in the middle, so if you like {\color{orange}$x_2$:}  Not to mention the flavor from the mesquite grill which is unlike anything else out there. {\color{orange}$x_3$:}  Went here with a couple of other people. {\color{orange}$x_4$:}  Perhaps they didn't finish constructing the place? {\color{orange}$x_5$:}  My friend who ordered the hot dog said the bun was hard, and he felt it was stale vs. being toasted. &        1 \\
 presum &  {\color{orange}$x_1$:}  I highly recommend JJ 's on Hayden ! ! ! !. {\color{orange}$x_2$:}  I noticed that a new Jimmy John 's had opened on Hayden in McCormick Ranch. {\color{orange}$x_3$:}  We used to order sandwiches a couple times a week at work in Seattle. {\color{orange}$x_4$:}  When I moved to Scottsdale about a year ago , I would make the drive to North Scottsdale ( 8 - 10 miles ) just for a delicious sandwich. &  {\color{orange}$x_1$:}  I split the an Arizona style and a Glendale style burger. {\color{orange}$x_2$:}  This restaurant just opened 10/21/11. {\color{orange}$x_3$:}  Gary also brought around a " Arizona " style burger that had been mis - ordered. {\color{orange}$x_4$:}  The Arizona burger was definitely the better of the two. {\color{orange}$x_5$:}  Gary hooked my wife up with their super - fire - burner - hot sauce , and while I ca n't do those types of things , my wife said it has great flavor and was indeed very hot. &        0 \\
     ig &                                                                                                                                   {\color{orange}$x_1$:}  I am a sandwich fan, and had heard about Jimmy John's for several years, but had never been able to stop and try one. {\color{orange}$x_2$:}  I recently moved to Scottsdale from Seattle and was pleased to know that there is a Jimmy John's just around the block from me. &                                                                                                                                                                                                          {\color{orange}$x_1$:}  I feel very strongly about supporting these types of family owned and local businesses, and I look forward to working my way across their menu. {\color{orange}$x_2$:}  I'm guessing the fry oil was fresh and super hot, because the shell of the chimi was perfectly toasted, flaky and wasn't greasy at all. &        1 \\
decsumnew111 &                                  {\color{orange}$x_1$:}  Thank you, Jimmy John's!  :) {\color{orange}$x_2$:}  It took everything inside of me not to walk back in and put them in their place. {\color{orange}$x_3$:}  Thank you Jimmy John's, for adding a little brightness to my day. {\color{orange}$x_4$:}  Freaky fast! {\color{orange}$x_5$:}  The kids pointed and laughed behind his back while mocking him as he walked away. &                                                                                                                                                                             {\color{orange}$x_1$:}  The chimi and burger were full sized, however I'm used to a bit more fries (and/or rings), but personally i'm trying to avoid the "super size" mentality, so it's fine by me. {\color{orange}$x_2$:}  Showing up at a new restaurant on opening day is a real treat because usually it's about the only time you'll see owners and managers. &        3 \\ \midrule
 &\includegraphics[width=\linewidth]{figs/intro/dist_118.pdf}&\includegraphics[width=\linewidth]{figs/intro/dist_146.pdf} & \\
 \bottomrule
    \end{tabular}
    \caption{Index 118 vs 146(better)}
    \end{table*}

\begin{table*}[h!]
    \centering
    \small
    
    \begin{tabular}{p{0.07\linewidth} | p{0.43\linewidth} | p{0.43\linewidth} | p{0.07\linewidth} }
        \toprule
        method &                                                                                                                                                                                                                                                                                                                                                                                                                                b1summary (better)  &                                                                                                                                                                                                                                                                                                                                                                                                                                                                               b2summary &  correct \\
 \midrule
        random &                                                                                {\color{orange}$x_1$:}  made food ! {\color{orange}$x_2$:}  Sorry guys, you need to step up your game to charge \$10 for a box of nothing. {\color{orange}$x_3$:}  We decided to give this place another try, 3 weeks later to see if they could improve. {\color{orange}$x_4$:}  I came here the second day it was open as ordered a small shawarma wrap. &                                                                                               {\color{orange}$x_1$:}  The flower added a spark of colour in the presentation but did not add anything to my tastebuds. {\color{orange}$x_2$:}  Red Bean Rice cake, Strawberry and chocolate mint. {\color{orange}$x_3$:}  rolls a try! {\color{orange}$x_4$:}  I would probably come back again if the queue at Sushi on Bloor is ridiculous. {\color{orange}$x_5$:}  it was soaked in. &        1 \\
        presum &                               {\color{orange}$x_1$:}  Ordered the shawarma boss and was GREAT !. {\color{orange}$x_2$:}  It was COLD compared to my boyfriend 's shawarma. {\color{orange}$x_3$:}  It has a great balance of vegetables , meat and rice ( Shawarma box ). {\color{orange}$x_4$:}  Amazing food , well done simple menu. {\color{orange}$x_5$:}  The shawarma is great here , in fact it 's my new favorite for shawarma. &                                                                                                                   {\color{orange}$x_1$:}  Sushi Combo ( \$ 9 ) is amazing value ... {\color{orange}$x_2$:}  5 pieces of sushi and a California roll with soup and salad and {\color{orange}$x_3$:}  that 's dinner pricing ! !. {\color{orange}$x_4$:}  a new Japanese restaurant just doing a soft opening in the Annex. {\color{orange}$x_5$:}  9 dollars for the Linerator roll , but &        1 \\
            ig &  {\color{orange}$x_1$:}  I don't recommend this place, unless you're into buying cold dry and flat shawarma. {\color{orange}$x_2$:}  Amazing food, well done simple menu. {\color{orange}$x_3$:}  The shawarma is great here, in fact it's my new favorite for shawarma. {\color{orange}$x_4$:}  In addition to my shawarma looking and tasting less than satisfactory, my boyfriend's shawarma was completely disproportionate to mine. &  {\color{orange}$x_1$:}  The service was friendly and efficient, but the food took forever to come! {\color{orange}$x_2$:}  All the specialty rolls are really good. {\color{orange}$x_3$:}  The Linerator roll is really, really delicious. {\color{orange}$x_4$:}  The miso soup that was included was really good, and the salad was just ok. {\color{orange}$x_5$:}  I was one of only 3 tables in the restaurant (which was mostly empty), and it took 25 minutes to get my rolls. &        0 \\
  decsumnew111 &                  {\color{orange}$x_1$:}  I was better off going to their competitor for a burrito next door. {\color{orange}$x_2$:}  Better than the other places up the road at Lawrence Ave. {\color{orange}$x_3$:}  There's better value for money there. {\color{orange}$x_4$:}  made food ! {\color{orange}$x_5$:}  I also called to put in a pick-up order (to cut down on time spent at the restaurant), but there was no answer. &                                                                                                                  {\color{orange}$x_1$:}  I opted for the sushi and sashimi lunch, which was 8 pieces of sashimi along with a california roll for \$9.95. {\color{orange}$x_2$:}  6th - Bacon dish with two components. {\color{orange}$x_3$:}  I can only give an honest based on what was plated and am sad to give this a one star at an outing full of great people and conversation. &        2 \\
 \bottomrule    \midrule
    &\includegraphics[width=\linewidth]{figs/intro/dist_103.pdf}&\includegraphics[width=\linewidth]{figs/intro/dist_319.pdf} & \\
    \bottomrule
    \end{tabular}
    \caption{Index 103 vs 319(better)}
\end{table*}

\begin{table*}[h!]\centering\small\begin{tabular}{p{0.07\linewidth} | p{0.43\linewidth} | p{0.43\linewidth} | p{0.07\linewidth}}
    \toprule
           method &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     b1summary &                                                                                                                                                                                                                                                                                                                                                                                                                                b2summary & correct \\
    \midrule
           random &                                      \textcolor{orange}{SS1:}  you sometimes get at other places. \textcolor{orange}{SS2:}  There was only ONE place that delivered sushi in my area \textcolor{orange}{SS3:}  Just opened. \textcolor{orange}{SS4:}  We ordered dumplings but nothing special. \textcolor{orange}{SS5:}  No big deal, but they packaged another roll I had ordered, with it. \textcolor{orange}{SS6:}  Too many good Chinese restaurants available to go back to a poor one. &  \textcolor{orange}{SS1:}  If you are looking for an authentic bagel, this is not the place to go. \textcolor{orange}{SS2:}  I do love this place. \textcolor{orange}{SS3:}  I frequently pick up the bucket o' bagels for the office, and you get two cream cheeses (shmears) with each bucket. \textcolor{orange}{SS4:}  Love those egg bagel sandwiches, the turkey sausage or the spinach mushroom swiss are the best in my opinion. &       0 \\
           presum &                                                                                                                            \textcolor{orange}{SS1:}  Menu is extensive with a mix of Japanese and Chinese foods. \textcolor{orange}{SS2:}  The rice is the WORST. \textcolor{orange}{SS3:}  House fried rice was tasty and not over oily. \textcolor{orange}{SS4:}  Its the type of rice you typically see in Mexican dishes and really weird to have in both the chinese food and the sushi. &                                             \textcolor{orange}{SS1:}  Chompies is about three stars on my list of bagel places but NY Bagels and Bialys is probably the closest thing I have had to real bagel since I have been out West. \textcolor{orange}{SS2:}  Einstein Bros Bagels in Tempe is my typical go - to breakfast spot. \textcolor{orange}{SS3:}  Einstein bagels are NOT real bagels , they are basically round bread. &       0 \\
               ig &                                                                      \textcolor{orange}{SS1:}  Worst egg roles I have ever tasted. \textcolor{orange}{SS2:}  Not very good. \textcolor{orange}{SS3:}  and I wont be going back. \textcolor{orange}{SS4:}  Fried rice was sticky and no taste. \textcolor{orange}{SS5:}  No beer but I will certainly return. \textcolor{orange}{SS6:}  Took a big chance and tried their yellowtail (hamachi) sushi and it was pretty good and made to order. &                                                                            \textcolor{orange}{SS1:}  Drip coffee that is the best in town, go with the bold European blend or the Vanilla blend. \textcolor{orange}{SS2:}  Love those egg bagel sandwiches, the turkey sausage or the spinach mushroom swiss are the best in my opinion. \textcolor{orange}{SS3:}  Great place for a smaller breakfast, and pretty great coffee as well. &       0 \\
     decsumnew111 &  \textcolor{orange}{SS1:}  Well I tried this place on a whim \textcolor{orange}{SS2:}  other reviews compared fried rice to mexican rice. \textcolor{orange}{SS3:}  I LOVE that they have a varied menu with sushi options. \textcolor{orange}{SS4:}  The Steamed Dumplings were tender and flavorful without the dipping sauce, General Tso seemed to be on the sweet side even though it's supposed to be spicy, and the Lo Mein was excessively oily, but overall the entrees tasted good. &                                                                                                           \textcolor{orange}{SS1:}  rug rat starts bumping into me. \textcolor{orange}{SS2:}  I love AZ but being from NYC, there is one thing that AZ doesn't do well and that is bagels. \textcolor{orange}{SS3:}  I frequently pick up the bucket o' bagels for the office, and you get two cream cheeses (shmears) with each bucket. &       3 \\
                  &                                                                                                                                                                                                                                                                                                                                                                                                                                   \includegraphics[width=\linewidth]{figs/intro/dist_117.pdf} &                                                                                                                                                                                                                                                                                                                                                                              \includegraphics[width=\linewidth]{figs/intro/dist_188.pdf} &         \\
    \bottomrule
    \end{tabular}
    \end{table*}
    

==> tables.tex <==

\begin{table}
    \centering

    \begin{tabular}{lrr}
        \toprule
        method &      MSE $\downarrow$ &  MSE v.s. \textbf{All} $\downarrow$  \\
        \midrule
        All & 0.146 & 0 \\\midrule
        BART & 0.499 & 0.316 \\
        PreSum & 0.487 & 0.296 \\ \midrule
            IG & 0.503 & 0.315 \\
        + sqrt length norm & 0.587 & 0.381 \\\midrule
        Attention & 0.646 & 0.409 \\
        + sqrt length norm & 0.696 & 0.439 \\ \midrule
        \multicolumn{3}{l}{\system ~ w/ ($\alpha$, $\beta$, $\gamma$)} \\ %
        (1, 0, 0) & 0.153 & 0.007 \\
        (0, 1, 0) & 0.494 & 0.412 \\
        (0, 0, 1) & 0.280 & 0.165 \\
        (1, 1, 0) & 0.149 & 0.010 \\
        (1, 0, 1) & 0.179 & 0.030 \\
        (0, 1, 1) & 0.330 & 0.259 \\
        (1, 1, 1) & 0.152 & 0.003 \\
        \bottomrule
    \end{tabular}
    \caption{MSE of model predictions based on summaries of different methods. \textbf{All} denotes using all reviews without summarization.
    }
    \label{tab:mse}
\end{table}

